Logic Blog 2023-2024

The logic blogs 2023 and 2024 have been joined. The present file contains a lot on particular classes of groups and their relationship with logic, as well as entries on ergodic theory and on foundations. There is also a bit on AI proving at the end.

==> sections2023/Nies_normaliser.tex <==
 \section{Kaplan, Nies,  Schlicht and others: closed subgroups of $\S$}
 
 We make some remarks on closed subgroups of $\S$. These are the automorphism groups of   structures with domain $\omega$. We in particular consider the following kind. 
 A closed subgroup $G$ of $\S$ is called \emph{oligomorphic} if it has only finitely many $n$-orbits, for each $n$. These are the automorphism groups of the $\aleph_0$-categorical structures with domain $\omega$.  We say that a topological  group $G$  is   \emph{quasi-oligomorphic} if it is in a topological group isomorphism with an oligomorphic group.  
 
 \subsection{The centre}

 
Let $G$ be a closed subgroup of $\S$.  For $p \in \omega$, by $k_p(G)$ we denote the number of  orbits  of the natural action of $G$  on $\omega^p$; such orbits will be   called $p$-orbits. (The parameter  $k_p(G)$ is denoted $F_p^*(G)$ in \cite{Cameron:90}.)  For $r \in \omega$ let $k_2(G,r)$ denote the number of $2$-orbits containing a  pair of the form $(r,t)$ (which only depends on the 1-orbit of $r$). 
 Suppose that $k_1(G) = n$ and let  $r_1, \ldots, r_n \in \omega$ represent the $1$-orbits.
 
 \begin{fact} $|C(G)| \le \prod_{i \le n} k_2(G, r_i)$. In particular, if $G$ is $1$-transitive then the size of the centre  is at most $k_2(G)$. \end{fact}
 
 \begin{proof} Write $C = C(G)$. 
 For any $r \in \omega$, and $c , d\in C $, if $cr \neq d r$ then $(r,cr)$ and $(r, dr)$ are in different $2$-orbits. Hence $|Cr| \le k_2(G,r)$.
 
 Consider now  the natural  left action $C \curvearrowright  \prod_i C   r_i$ (Cartesian product of sets). If $c , d\in C $ are distinct then   $c g r_i \neq d g r_i$ for some $i$ and $g \in G$, so that $c r_i \neq d r_i$. Hence $|C| \le \prod_{i \le n} |C \cdot r_i|$. This shows the required bound. \end{proof}
 
 
 Greg Cherlin suggested another way to prove that  for oligomorphic $G$ the centre $C(G)$  is finite   (but without an explicit bound on its size).  We may suppose $G = \Aut(M)$ for an  $\aleph_0$-categorical structure $M$  with domain~$\omega$. Note that $\Phi \in \Aut(M)$ is definable as a  binary relation on $M$ iff $\Phi$ is invariant under the natural action of  $G$ on $M$, i.e., $\Phi \in C(G)$.  Since there are only finitely many definable binary relations, $C(G)$ is finite. 
 
 
  We consider   examples of oligomorphic groups $G$ with a nontrivial centre.  
  
 \n  1. For any finite abelian group $A$, the natural action of $A \times \S$ on $A \times \omega$ yields an 1-transitive oligomorphic group with centre $A$. The number of $2$-orbits is at least $|A|$ because $(an, a'n') \approx (bm, b'm')$ implies that $a-b = a'-b'$.  (In fact it is $2 |A|$.) 
 
 \n 2. Let $M_1$ be the structure with one equivalence relation $E$ that has all classes of size $2$; say,    for $x,y \in \omega$
 %
\bc  $ x E y \lra  x \mod 2 = y \mod 2$.  \ec
Write $C_k = \ZZ/ k\ZZ$.  We have $ G_1 := \Aut(M_1) = C_2 \wr \S$, where $\wr$ denotes the unrestricted wreath product.   Here $\S$ is viewed with its natural action on  $\omega$; so $G $ is an extension of $L= C_2^\omega$ by $\S$ with $\S$ acting by $\phi \cdot f = f \circ \phi$, for $f\in L$.  (Note that $L$ is the automorphism group of the structure where the individual equivalence classes are now  distinct unary predicates.  $G$ is the normaliser of $L$ in $\S$.)   The centre $C(G)$ consists of the identity and the  automorphism that maps  each element to the other one in its $E$ class.  The centre of $G/C(G)$ is trivial. 
 
 \n 3. Let $M_2$ be the structure with   equivalence relations $E \sub F$ such that each $E$-class has size 2 and each $F$-class has size 4. Then  the automorphism group of a single $F$-class is $C_2 \wr C_2$, and hence $G_2 := \Aut (M_2)  = (C_2 \wr C_2) \wr \S)$.    As before,  the centre $C(G_2)$ consists of the identity and the  automorphism  that switches each element in its $E$ class.  We have $G_2 / C(G_2)  \cong G_1$. 
 
 Similarly,   for each $n$ there is an oligomorphic group $G_n = \Aut(M_n)$ with a  chain of $n$ higher centres.  
 
 \subsection{The central quotient} The main purpose in this section is to show that \emph{for oligomorphic $G$, the central quotient $G/C(G)$ is quasi-oligomorphic}. Some facts needed along the way hold in more generality.
 
 Suppose a group $G$ acts on a set $X$ and $N \trianglelefteq G$. Write $\sim_N$ for the orbit equivalence relation of the subaction of $N$. Note that $G$ acts naturally on $X/\sim_N$ via $g\cdot [x] = [g\cdot x]$ (where $[x]$ is the $\sim_N$ class of $x$).  Since elements of $N$ act as the identity, $G/N$ acts on $X / \sim_N$. 
 
 Suppose now $G$ initially acts faithfully on a set $Y$, say $Y = \NN$. Let $X =  Y \times Y$ and let  $G$ act on $X$ by the usual diagonal action. Let $N= C(G)$.  
 
 \begin{fact} The action of $G /C(G)$ on $X / \sim_{C(G)}$ is faithful. \end{fact}
 
 To see this, suppose $g \not \in N =C(G)$. So grab $\eta \in G$ such that \bc $ (g \eta) \cdot w \neq (\eta g) \cdot w$. \ec  Let $w'= \eta \cdot w$.  Then $ g \cdot (w,w') \not \sim_N (w,w')$,  because any element $h $ of $G$ such that $h \cdot (w,w') = g \cdot (w,w')$ satisfies $(h \eta) \cdot w \neq (\eta h) \cdot w$, so that $h \not \in C(G)$. 
 
 
 We now switch to topological setting. Given  a Polish group $H$  with a faithful  action $\gamma \colon H \times V \to V$, say  for a  countable set $V$,  we obtain a monomorphism $\Theta_\gamma \colon H \to S_V$ given by $\Theta_\gamma(g)(k)= \gamma(g,k)$. A Polish group action is continuous iff it is separately continuous (i.e. when one argument is fixed). In the case of an action on countable $V$ (with the discrete topology), the latter condition  means that  
 
 \bi \item[(a)] for each $k,n \in V$, the set $\{ g \colon \gamma(g,k)=n\}$ is open. \ei
 
 
 So $\gamma$ is continuous iff $\Theta_\gamma$ is continuous. 

\begin{definition} 
We say that a faithful  action $\gamma \colon H \times V \to V$   is \emph{strongly continuous} if the embedding $\Theta_\gamma$ is topological. 
\end{definition} 

Equivalently, the action is continuous,  and for each neighbourhood $U$ of $1_H$, also $\Theta_\gamma(U)$ is open, namely,   

 \bi \item[(b)]
for each neighbourhood $U$ of $1_H$, there is finite set $B \sub V$  such that $\fa k \in B \, \gamma(g,k) = k$ implies $g \in U$.  \ei Since $H$ is Polish, strong continuity of the action  implies that $H$  is topologically isomorphic  via $\Theta_\gamma$ to a closed subgroup of $S_V$ (see e.g.\  \cite[Prop.\ 2.2.1]{Gao:09}).
 
 Now consider the case that $Y = \NN$ and  $G$ is a closed subgroup of $\S$. Since $C(G)$ is closed, $H= G/C(G)$ is naturally a Polish group via  the quotient topology:  for $C \le U \le G$, the   subgroup $U/C \le H$ is declared to be open iff $U$ is open in $G$.  (See e.g.\  \cite[Prop.\ 2.2.10]{Gao:09}.)
 
 
 
Let  $X = Y \times Y$ as above. Suppose that $V:= X/\sim_{C(G)}$ is infinite (e.g.\ when $C(G)$ is finite),  so through the action $\gamma$ above we obtain  an (algebraic) embedding $\Theta_\gamma$ of $G/C(G)$ into $S_V$ (which can be identified with $\S$).  
 
 \begin{claim}  \label{cl:1tr} Suppose that $G$ is a closed subgroup of $\S$ that  acts 1-transitively on $Y = \NN$. Suppose that   $C(G)$ is finite. Then $\Theta_\gamma \colon G/C(G) \to S_V$  is a topological embedding. \end{claim}
 \begin{proof} 
 We check the conditions (a) and (b) above.  
 
 \medskip 
 
\n  (a) Suppose that $k = [(w_0, w'_0)], n  = [(w_1, w'_1)]$. Then $\gamma(g,k)=n$ iff there are $(v_0, v'_0) \sim_C (w_0, w'_0)$ and  $(v_1, v'_1) \sim_C (w_1, w'_1)$ such that $g \cdot v_0 = v_1$ and $g \cdot v'_0 = v'_1$. Since $C(G)$ is finite this condition is open.
 
 
 \medskip 
 \n  (b) An open  neighbourhood   of  $1_{G/C}$ has the form $U/C$ wherewhere $U \sub G$ is   open   and $C \le U$.   By definition of the topology on $G$, we may assume that  $U = G_{R} C$ for some finite $R \sub Y$ (as usual $G_R$ is the pointwise stabiliser). Let $B = (R \times R) / \sim_C$. Consider $g = pC \in H$, where $p \in G$. 
 
 Suppose that  $\fa k \in B \, \gamma(g,k) = k$. This means that for each $u,v \in R$, there is a $c_{u,v} \in C$ such that $p \cdot  (u,v) = c_{u,v} \cdot  (u,v)$. Since $G$ acts faithfully and 1-transitively on $Y$, for each $c,d \in C$, and each $y \in Y$, $c\cdot  y = d \cdot y$ implies that $c=d$. Therefore given another pair $r,s \in R$, $c_{u,v} = c_{u,s} = c_{r,s}$. Let $c$ be this unique witness. Then $p \cdot u = c \cdot u$ for each $u \in R$, hence  $p \in G_R C$ and therefore $g \in U/C$.
 \end{proof}
 
 
 \begin{thm} Let   $G$ be oligomorphic.  The central quotient $G/C(G)$ is quasi-oligomorphic (i.e.\ homeomorphic to an oligomorphic group). \end{thm}
 \begin{proof} 
 It is   known (as pointed out to us by Todor Tsankov) that we may assume $G$ is 1-transitive.  To see this,  one shows that there is an open subgroup $W$ such that the left translation action $\gamma \colon G\curvearrowright G \backslash W$  of  $G$ on the left cosets of $W$ is faithful and oligomorphic, and the corresponding embedding  into a copy of $\S$ is topological. To get $W$,   let $x_1, \ldots, x_k \in \omega$ represent the 1-orbits of $G$. Let $W$ be the pointwise stabiliser of $\{x_1, \ldots, x_k\}$. If $g \in G - \{1\}$ then there is $p \in G$ and $i \le k$ such that $g \cdot (p \cdot x_i) \neq p\cdot x_i$. So $p^{-1} g p \not \in W$, and hence $g \cdot  p W \neq pW$.   So the action is faithful. The rest is routine using (a) and (b) above. 
 
 Now we can apply Claim~\ref{cl:1tr}, recalling that $C(G)$ is finite. 
 \end{proof} 
 
 
 
 For any closed subgroup $G = \Aut(M) $ of $\S$  the higher centres  are normal, so their orbit equivalence relations are $G$-invariant. If $G$ is oligomorphic they are   definable in $M$. Hence the progression of higher centres has to stop at a finite stage for each oligomorphic group $G$.  

   \subsection{Conjugacy}
 We show that conjugacy of oligomorphic  groups is smooth.  For a closed subgroup $G$ of $ \S$, let $V_G$ denote the orbit equivalence structure. For each $n$ this structure has a $2n$-ary relation symbol, denoting the orbit relation on $n$-tuples. (One could require here that the tuples have distinct elements.)
 
 
 The following fact     holds for non-Archimedean groups in general.

 \begin{fact} \label{fact:conj}Let $G, H$ be   closed subgroups of $\S$. 
 
 \bc $G, H$ are conjugate via $\alpha$ $\LR$ $V_G \cong V_H$ via $\alpha$. \ec
 \end{fact}
 
 \begin{proof}
 \rapf  Immediate.
 
 \lapf Let $M_G$ be the canonical structure for $G$;  namely there are $k_n \le \omega$ many $n$-ary relation symbols, denoting the $n$-orbits. Let $M_H$ be the structure in the same language where the $n$-equivalence classes of $V_H$ are named so that $\alpha$ is an isomorphism $M_G \cong M_H$. Clearly $G= \Aut(M_G)$ and   $H = \Aut(M_H)$. Further, $\alpha^{-1} \Aut(M_H) \alpha = \Aut(M_G)$.
 \end{proof}


 \begin{prop} Conjugacy of oligomorphic groups is smooth. \end{prop}
\begin{proof}   The map $G \to V_G$ is   Borel because we can in a Borel way find a countable dense subgroup of $G$, which of course  has the same orbits.  Now apply Fact~\ref{fact:conj}.  For  countable structures $S$ in  a fixed  language,   mapping   $S$ to its theory $\text{Th}(S)$ is Borel.   Since the theory can be seen as  a real, for $\omega$-categorical structures,  this shows smoothness. 
\end{proof}

For corresponding structures $A,B$ with $\Aut(A) = G,\Aut(B) = H$, conjugacy of $G,H$ via $\alpha$ means that $\alpha( A) $ and $B$ have the same definable subsets. To see this, consider the case that $A$ is the canonical structure for $G$. 


We note the following topological variation  of Prop~\ref{prop:Sn_normaliser}. The   notation is  introduced   above.

\begin{prop}  (i) $\Aut(V_G)$ equals  the normaliser $N_G$  of $G$  in $\S$.

(ii) If $G$ is oligomorphic then $N_G /G$ as a topological group is profinite.  \end{prop}

\begin{proof}
\n (i) 
\n $\sub:$  Let $\alpha \in \Aut(V_G)$, $\beta \in G$. Clearly $\alpha$ maps $n$-orbits to $n$-orbits, so  $\alpha(M_G)$ is a renumbering of the named $n$-orbits in $M_G$. Therefore $\beta^\alpha \in \Aut(M_G) =G$. 

\n $ \supseteq:$  Let $V$ be an $n$-orbit, and let $\alpha \in  N_G$.  If $r, s \in \NN^n$ and $r,s \in \alpha(V)$, choose $\beta \in G$ such that $\alpha \beta \alpha^{-1} (r) =s$. So $\alpha(V) $ is contained in an $n$-orbit $W$. By a similar argument, $\alpha^{-1}(W)$ is contained in an $n$-orbit. Therefore $\alpha(V) = W$ is an $n$-orbit.  Hence $\alpha \in \Aut(V_G)$.


\n (ii). Let $k_n$ be the number of $n$-orbits of $G$.  Define a continuous homomorphism $\Theta: \Aut(V_G) \to \prod_n S_{k_n}$ by $\Theta(\alpha)= f$ if  $f(n)$ is the finite permutation describing the way $\alpha$ permutes $n$-orbits (numbered in some way). Clearly $G$ equals  the kernel of $\Theta$, and $\Theta/G$ is therefore a topological embedding. Since the range is compact, its inverse is also continuous. 
A closed subgroup of a profinite group is again profinite.
\end{proof} 

The converse of (ii) may fail: $N_G/G$ can be profinite, and even trivial, without $G$ being oligomorphic. For instance, there is a countable maximal-closed subgroup of $\S$, e.g.\ $AGL_n(\mathbb Q)$, the automorphism group of the structure $\mathbb Q^n$, $n \ge 2$ with the ternary function $f(x,y,z) = x+y-z$ (Kaplan and Simon). This structure is not $\omega$-categorical. 

 We don't know at present whether every profinite group occurs that way.
 
 

\subsection{$\omega$-categorical  structures with essentially finite language} 
One says that a structure $M$ has essentially finite language if $M$ is interdefinable with a structure $\wt M$ over a language in a finite signature.   (Interdefinable means same domain and same definable relations.). We present a basic fact that  can be used to obtain an oligomorphic group that is not isomorphic to   the automorphism group of such an $\omega$-categorical structure.


\begin{lemma} The following are equivalent  for a countable structure $M$.
\bi
\item[(i)] $M$ is interdefinable with a structure $N$ in  finite language with maximum arity $k$, and quantifier elimination.

\item[(ii)] $M$ is $\omega$-categorical, and for each  $n \ge k$, each $n$-orbit of $M$ is given by its projections to $k$-orbits. 
\ei
\end{lemma}
\begin{proof} (ii) implies  (i): Let  $G = \Aut (M)$, and let $N$ be the orbit structure of $M$. Thus,  $N$ is like     $V_G$ above but has an  $n$-ary predicate for each $n$-orbit. (Note that $N$ is a Fraisse limit. $V_G$ is a reduct of $N$, and as in the  finite case above its automorphism group  is the normaliser of $G$.)

(i) implies  (ii): Clearly $N$ is $\omega$-categorical, as there are only finitely many $n$ types for each $n$. 
Each formula $\phi$  in $n\ge k$ variables is a Boolean combination of q-free formulas in $\le k$ variables. If $\phi$ describes an $n$-orbit we can assume it is a conjunction of such formulas. A formula in $k' \le k$ variables describes a finite union of $k'$-orbits. Hence the $n$-orbit is given by its projections: if two $n$ tuples have are in the same projection orbits then both or none satisfy $\phi$.


\end{proof}


==> sections2023/Schlicht_meetgroupoid.tex <==



\section{Nies and Schlicht: The meet groupoid of an oligomorphic group}
\begin{definition} 
\label{def:MeetGroupoid} A \emph{meet groupoid} is a groupoid  $(H, \cdot , {}^{-1})$ that is also a meet semilattice  $(H, \wedge  ,\ES)$ with least element $\ES$, and 
%and letting the operation $\cdot$ have preference over $\cap$,
  satisfies the following conditions. Let $\sqsubseteq$ denote the induced partial order $A\sqsubseteq B :\Leftrightarrow A\wedge B=A$.

\begin{enumerate} 
\item 
(least element) 
$\ES$ is an idempotent such that $\ES \cdot A$ and $A \cdot \ES$ are only defined for $A = \ES$. 

\item
(compatibility)
For all idempotents $U,V\neq\emptyset$, $U  \wedge V \neq \ES$. 
%\item 
%$\emptyset^{-1}=\emptyset=\emptyset \cdot\emptyset$, and $\emptyset \cdot A$ and $A\cdot \emptyset$ are undefined for each $A=\emptyset$, 

\item 
(monotonicity of inverse)
$A\sqsubseteq B$ $\Leftrightarrow A^{-1} \sqsubseteq B^{-1}$. 

\item 
If $A_i \cdot B_i$ are defined for $i=0,1$ and $A_0\cap A_1\neq \emptyset \neq B_0\cap B_1$, then 
$$ (A_0\cap A_1)  \cdot (B_0\cap B_1) = (A_0\cdot B_0) \cap (A_1 \cdot B_1). $$ 
\end{enumerate} 
\end{definition} 

 In the following let $G \le_c \S$ be an oligomorphic closed subgroup of the symmetric group $\S$. Let   $\+ W(G)$ be the collection of    cosets of open subgroups of $G$ and $\ES$ with inclusion. This   is a meet groupoid.  

 
% \subsection{} 
 \subsection{A model theoretic view of $\+ W(G)$}
  \subsubsection*{The structure of imaginaries for an $\omega$-categorical structure $M$}
 Let $M$ be a countable 
 %$\omega$-categorical 
structure with domain $\omega$. By ``definable" we mean first-order definable in $M$  without parameters. The structure $M^{eq}$ of imaginaries over $M$, going back to Poizat and Shelah,   has sorts $S= D/E$ for any $k \ge 1$,  nonempty  definable  $D \sub M^k$, and definable equivalence relation $E$ on $D$. We will use $\aaa, \beta, \ldots$ for elements of $M^{eq}$.  The atomic   relations of $M^{eq}$  are the  atomic  relations of the given structure $M$ (viewed as relations on the  ``home sort" $M$), as well as the graphs of the projections $D \to S=D/E$ for each sort $S$. 
 
 In a many-sorted structure, each definable relation is a subset of $\prod_{i< n} S_i$ for sorts  $S_0, \ldots, S_{n-1}$.  The   definable relations are given  as usual via   formulas in the   first-order logic in the corresponding signature  with variables for each sort.  Extending the usual  definition of algebraic/definable closure to a many-sorted structure is no problem. We note that assuming $M$ is $\omega$-categorical, $\text{acl}(A)  \cap S$ is finite for each finite $A \sub M^{eq}$ and  each sort $S$. 
 
 \subsubsection*{Open subgroups as stabilisers of imaginaries}
  It is well-known that   $G= \Aut(M_G)$ for an $\omega$-categorical relational structure $M_G$ that has a $k$-ary relation for each $k$-orbit of $G$. In this context one says that $M_G$ is a canonical structure for $G$; it is unique up to renaming the $k$-orbits, for each $k$.  Letting $G$ act on $M^{eq}$ in the canonical way, we have  the following well known fact  due to Ahlbrandt/Ziegler \cite{Ahlbrandt.Ziegler:86}  (see Theorem 2.7 in   \href{http://wwwf.imperial.ac.uk/~dmevans/Bonn2013_DE.pdf}{ David Evans' 2013  notes}).
  $U \le_o G$ denotes that $U$ is an open subgroup of $G$. 
  
  
\begin{fact} \label{fac1}  $U \le_o G \LR U = G_{\aaa}$ for some $\aaa \in M^{eq}$. 
Moreover, for any $\bar{a}$ with $G_{\bar{a}}\subseteq U$, $\alpha$ can be chosen to be of the form $\bar{a}/E$, where $E$ is some definable 
\iffalse 
{\color{red} without parameters? } 
\fi 
equivalence relation. 
\end{fact}
 
 \begin{proof} 
 For the implication ``$\LA$", suppose that $\aaa \in D/E$ as above. We have $\aaa = \ol a  /E$ for some $\ol a \in D$. The pointwise stabiliser $G_{\ol a}$ is open by definition of the topology of $G$, and is contained in $G_\aaa$. So $G_\aaa$ is open as well. 
 
 
  For the implication ``$\RA$",  pick $\ol a$ such that  $G_{\ol a}\sub U$. Let $D = G\cdot \ol a$, and define an  equivalence relation $E$ on $D$ by 
  \[  h \ol a E g  \ol a  \lra g^{-1}h \in U.\]
  Let $\alpha$ be the equivalence class of $\ol a$. 
  Then we have $G_\aaa = U$, because $g(\aaa) = \aaa \lra g(\ol a ) E \ol a \lra g \in U$. 
\end{proof} 

Note that the orbit equivalence relation $E_{G_{\alpha}}$ on $M^k$ of an open subgroup $G_{\alpha}$ is definable from $\alpha$, since $\bar{c} E_{G_{\alpha}} \bar{d}$ if and only if for some $\bar{a}, \bar{b}\in\alpha$, $\bar{a}^\smallfrown \bar{c}$ and $\bar{b}^\smallfrown \bar{d}$ have the same type. 

 We discuss a model theoretic characterisation (i)  of the containment relation between open  subgroups of $G$. This has a surprising consequence (ii) for the lattice of open subgroups.
 
 
  \begin{fact}  \label{fac2}\ 
  
  
  (i) $G_\aaa \sub G_\beta \LR \beta \in \text{dcl}(\aaa)$.


(ii) Each open  subgroup $U$ is contained in  only finitely many open subgroups.
  
 \end{fact}
 \begin{proof}
 (i) The implication ``$\LA$'' is immediate. For ``$\RA$", suppose $\aaa = \ol a /E$ and $\beta = \ol b /F$ as above. Then $h \ol a  E g \ol a  \lra g^{-1}h \in G_\alpha$  and similarly for $\ol b, F$ and $G_\beta$. 
 Let $R=  G \cdot \la \ol a , \ol b\ra$, and note that $R$ is a left invariant, and hence  definable, relation. 
 
\iffalse 
 {\color{red} improve this} 
\fi 

 Since $G_\alpha \sub G_\beta$, 
 %and the orbit equivalence relation of $G_{\alpha}$ is definable from $\alpha$, 
 $\beta$ is  the unique equivalence class of $F$ containing $\bar{c}$ for some $\langle \bar{b},\bar{c}\rangle \in R$ with $\bar{b}\in \alpha$. 
Hence $\beta \in \text{dcl}(\aaa)$. 
 
 (ii) If $U \sub V$ where $U = G_\aaa$, $\aaa = \ol a/E$,   by \cref{fac1}  we have  $V = G_\beta $ for some imaginary $\beta = \ol a /F$, and $E \sub F$. So the number of open subgroups containing $U$ is bounded by the number of definable equivalence relations on $G\ol a$ containing $E$.  
 \end{proof}


\iffalse 
 {\color{red} Continue here} 
\fi 


 There is a natural generalisation of (i), proved in the same fashion. For $\aaa_1, \ldots, \aaa_k, \beta \in M^{eq}$, one has \bc $\bigcap_iG_{\aaa_i} \sub G_\beta \LR \beta \in \text{dcl}(\aaa_1, \ldots, \aaa_l)$. \ec


For $\omega$-categorical structures $M$ letting $G= \Aut(M)$, the usual definition in model theory of weak elimination of imaginaries 
\iffalse 
 {\color{red} Cite definition of WEI from [Tent, Ziegler: A course in model theory, Definition 8.4.9.]} 
\fi 

can be rephrased as follows: \bc $G_{(A\cap B)} = \la G_{(A) },  G_{(B)} \ra_{gp}$, \ec
where $A,B$ range over  finite algebraically closed subsets of $M$.
\begin{prop} TFAE for $G$, $M=M_G$ as above

\bi \item[(i)] $M$ has weak elimination of imaginaries

\item[(ii)]  For each $U \le_o G$ there is a sort $D/E$ where $D = G\cdot \ol a$ is a $k$-orbit,  $U$ is the stabiliser of $\ol c/E$, and  each $E$-class has the same finite cardinality $|U\colon G_{(\ol a)}|$.

\item[(iii)] Each $U \le_o G$ contains a subgroup $G_{\ol a}$ of finite index, where $\ol a \in M^r$ for some $r$.

\item[(iv)] For each $U \le_o G$ there is $\ol b \in M^s$ for some $s$ such that $G_{(\ol b)}\sub U \sub G_{\{b_1, \ldots , b_s\}}$ (the Galois sandwich condition). 
\ei
\end{prop}


\begin{proof} (iv)$\to$ (iii) clearly we have $|  U\colon G{(\ol b)}| \le |G_{\{b_1, \ldots , b_s\}}  \colon G{(\ol b)}| \le s!$

(iii)$\to$ (ii)\\ 

\iffalse 
 {\color{red} Add this proof} 
\fi 
\end{proof}


%%%%%%%%%%%%%%
 \subsubsection{Open cosets}
 
 For imaginaries $\aaa_0, \aaa_1$ of the same sort, let 
 \[G_{\aaa_0 \mapsto \aaa_1} = \{ g \in G \colon g(\aaa_0)= \aaa_1\}. \] 
 In particular, $G_{\aaa\mapsto \aaa} = G_\aaa$. Clearly $G_{\aaa_0 \mapsto \aaa_1}$ is a right coset of $G_{\aaa_0}$ and a left coset of $G_{\aaa_1}$. Also $G_{\aaa_1 \mapsto \aaa_0}= G_{\aaa_0 \mapsto \aaa_1}^{-1}$. We extend \cref{fac2}(i). 
 
   \begin{fact}  \label{fac3}
  
       $G_{\aaa_0 \mapsto \aaa_1}=:A  \sub B:= G_{\beta_0 \mapsto \beta_1}  \LR $
       
       \hfill $A = \ES \vee \beta_i \in \text{dcl}(\aaa_i)$ ($i=0,1)$ via the same formula. \end{fact}
  \begin{proof}
 (i) The implication ``$\LA$'' is again  immediate. For ``$\RA$", suppose $\aaa_i = \ol a_i /E$ and $\beta_i = \ol b_i /F$ as above. Since $G_{\aaa_0} \sub G_{\beta_0}$, as before we have $\beta_0 \in \text{dcl}(\aaa_0)$, say via formula $\phi(\ol x, \ol y)$. 
 We may assume $A \neq \ES$, that is there is $g\in G$ with $g (\aaa_0) = \aaa_1$. Then $g (\beta_0) = \beta_1$. Hence $\beta_1 \in \text{dcl}(\aaa_1)$ via $\phi$. \end{proof}
 
 
 
 
 \subsubsection{Meet groupoid operations}
 
 

\iffalse 
\ \\ 
{\color{red} Goal: define the meet groupoid directly from the model (not from the automorphism group)\\ 
\ \\ 
What do we want to use this for? \\ 
Maybe we want to show directly that bi-interpretable $M$, $N$ define the same meet groupoids.\\ 
\ \\ 
Motivation: model theoretic version of meet groupoid\\ 
\ \\ 
New proof of results in paper Nies Schlicht \\ 
\ \\ 
Useful for outer automorphism group? 
}  


\bigskip 
{\color{blue} 
Andre's notes 15 May: \\ 
\ \\ 
Given G= Aut(M).\\ 
Goal: understand Out(G) model theoretically.\\ 
\ \\ 
To do so, think of elements of Aut(G) as self-BIs up to homotopy, as in A/Z. They can be studied modeltheoretically using W(M), the structure of equivalence classes of (certain pairs of) $M^{eq}$. It is likely that Inn(G) can be characterized as bi-definability
} 

\fi 




 
 
 

==> sections2023/backup_meetgroupoid.tex <==



\section{Nies and Schlicht: The meet groupoid of an oligomorphic group}
\begin{definition} 
\label{def:MeetGroupoid} A \emph{meet groupoid} is a groupoid  $(H, \cdot , {}^{-1})$ that is also a meet semilattice  $(H, \wedge  ,\ES)$ with least element $\ES$, and 
%and letting the operation $\cdot$ have preference over $\cap$,
  satisfies the following conditions. Let $\sqsubseteq$ denote the induced partial order $A\sqsubseteq B :\Leftrightarrow A\wedge B=A$.

\begin{enumerate} 
\item 
(least element) 
$\ES$ is an idempotent such that $\ES \cdot A$ and $A \cdot \ES$ are only defined for $A = \ES$. 

\item
(compatibility)
For all idempotents $U,V\neq\emptyset$, $U  \wedge V \neq \ES$. 
%\item 
%$\emptyset^{-1}=\emptyset=\emptyset \cdot\emptyset$, and $\emptyset \cdot A$ and $A\cdot \emptyset$ are undefined for each $A=\emptyset$, 

\item 
(monotonicity of inverse)
$A\sqsubseteq B$ $\Leftrightarrow A^{-1} \sqsubseteq B^{-1}$. 

\item 
If $A_i \cdot B_i$ are defined for $i=0,1$ and $A_0\cap A_1\neq \emptyset \neq B_0\cap B_1$, then 
$$ (A_0\cap A_1)  \cdot (B_0\cap B_1) = (A_0\cdot B_0) \cap (A_1 \cdot B_1). $$ 
\end{enumerate} 
\end{definition} 

 In the following let $G \le_c \S$ be an oligomorphic closed subgroup of the symmetric group $\S$. Let   $\+ W(G)$ be the collection of    cosets of open subgroups of $G$  together with $\ES$. This   is a meet groupoid.  

 
% \subsection{} 
 \subsection{A model theoretic view of $\+ W(G)$}
  \subsubsection*{The structure of imaginaries for an $\omega$-categorical structure $M$}
 Let $M$ be a countable $\omega$-categorical structure with domain $\omega$. By ``definable" we mean first-order definable in $M$  without parameters. The structure $M^{eq}$ of imaginaries over $M$, going back to Poizat and Shelah,   has sorts $S= D/E$ for any $k \ge 1$,  nonempty  definable  $D \sub M^k$, and definable equivalence relation $E$ on $D$. We will use $\aaa, \beta, \ldots$ for elements of $M^{eq}$.  The atomic   relations of $M^{eq}$  are the  atomic  relations of the given structure $M$ (viewed as relations on the  ``home sort" $M$), as well as the graphs of the projections $D \to S=D/E$ for each sort $S$. 
 
 In a many-sorted structure, each definable relation is a subset of $\prod_{i< n} S_i$ for sorts  $S_0, \ldots, S_{n-1}$.  The   definable relations are given  as usual via   formulas in the   first-order logic in the corresponding signature  with variables for each sort.  Extending the usual  definition of algebraic/definable closure to a many-sorted structure is no problem. We note that $\text{acl}(A)  \cap S$ is finite for each finite $A \sub M^{eq}$ and  each sort $S$.  
 
 \subsubsection*{Open subgroups as stabilisers of imaginaries}
  It is well-known that   $G= \Aut(M_G)$ for an $\omega$-categorical relational structure $M_G$ that has a $k$-ary relation for each $k$-orbit of $G$. In this context one says that $M_G$ is a canonical structure for $G$; it is unique up to renaming the $k$-orbits, for each $k$.  Letting $G$ act on $M^{eq}$ in the canonical way, we have  the following well known fact  due to Ahlbrandt/Ziegler \cite{Ahlbrandt.Ziegler:86}  (see detail in   \href{http://wwwf.imperial.ac.uk/~dmevans/Bonn2013_DE.pdf}{ David Evans' 2013  notes}).
\begin{fact} \label{fac1}  $U \le_o G \LR U = G_{(\aaa)}$ for some $\aaa \in M^{eq}$. \end{fact}
 
 
 For the implication ``$\LA$", suppose that $\aaa \in D/E$ as above. We have $\aaa = \ol a  /E$ for some $\ol a \in D$. The pointwise stabiliser $G_{\ol a}$ is open by definition of the topology of $G$, and is contained in $G_\aaa$. So $G_\aaa$ is open as well. 
 
 
  For the implication ``$\RA$",  pick $\ol a$ such that  $G_{(\ol a)}\sub U$. Let $D = G\cdot \ol a$, and ``well-define" an  equivalence relation $E$ on $D$ by 
  \[ E g \ol a h \ol a  \lra g^{-1}h \in U.\]
  Then we have $G_\aaa = U$, because $g(\aaa) = \aaa \lra g(\ol a ) E \ol a \lra g \in U$. 
  
 We discuss a model theoretic characterisation (i)  of the containment relation between open  subgroups of $G$. This has a surprising consequence (ii) for the lattice of open subgroups.
 
 
  \begin{fact}  \label{fac2}
  
  
  (i) $G_\aaa \sub G_\beta \LR \beta \in \text{dcl}(\aaa)$.


(ii) Each open  subgroup $U$ is contained in  only finitely many open subgroups.
  
 \end{fact}
 \begin{proof}
 (i) The implication ``$\LA$'' is immediate. For ``$\RA$", suppose $\aaa = \ol a /E$ and $\beta = \ol b /F$ as above. Then $E g \ol a h \ol a  \lra g^{-1}h \in U$  and similarly for $\ol b, F$ and $V$. Let $R=  G \la \ol a , \ol b\ra$, and note that $R$ is a left invariant, and hence  definable, relation. Since $U \sub V$ we have  $\beta \in \text{dcl}(\aaa)$ via $R$. 
 
 (ii) If $U \sub V$ where $U = G_\aaa$, $\aaa = \ol a/E$,   by the proof of  \cref{fac1}  we have  $V = G_\beta $ for some imaginary $\beta = \ol a /F$, and $E \sub F$. So the number of open subgroups containing $U$ is bounded by the number of definable equivalence relations on $G\ol a$ containing $E$.  
 \end{proof}
 
 There is a natural generalisation of (i), proved in the same fashion. For $\aaa_1, \ldots, \aaa_k, \beta \in M^{eq}$, one has \bc $\bigcap_iG_{\aaa_i} \sub G_\beta \LR \beta \in \text{dcl}(\aaa_1, \ldots, \aaa_l)$. \ec


For $\omega$-categorical structures $M$ letting $G= \Aut(M)$, the usual definition in model theory of weak elimination of imaginaries can be rephrased as follows: \bc $G_{(A\cap B)} = \la G_{(A) },  G_{(B)} \ra_{gp}$, \ec
where $A,B$ range over  finite algebraically closed subsets of $M$.
\begin{prop} TFAE for $G$, $M=M_G$ as above

\bi \item[(i)] $M$ has weak elimination of imaginaries

\item[(ii)]  For each $U \le_o G$ there is a sort $D/E$ where $D = G\cdot \ol a$ is a $k$-orbit,  $U$ is the stabiliser of $\ol c/E$, and  each $E$-class has the same finite cardinality $|U\colon G_{(\ol a)}|$.

\item[(iii)] Each $U \le_o G$ contains a subgroup $G_{\ol a}$ of finite index, where $\ol a \in M^r$ for some $r$.

\item[(iv)] For each $U \le_o G$ there is $\ol b \in M^s$ for some $s$ such that $G_{(\ol b)}\sub U \sub G_{\{b_1, \ldots , b_s\}}$ (the Galois sandwich condition). 
\ei
\end{prop}


\begin{proof} (iv)$\to$ (iii) clearly we have $|  U\colon G{(\ol b)}| \le |G_{\{b_1, \ldots , b_s\}}  \colon G{(\ol b)}| \le s!$

(iii)$\to$ (ii)
\end{proof}


%%%%%%%%%%%%%%
 \subsubsection{Open cosets}
 
 For imaginaries $\aaa_0, \aaa_1$ of the same sort, let 
 \[G_{\aaa_0 \mapsto \aaa_1} = \{ g \in G \colon g(\aaa_0)= \aaa_1\}. \] 
 In particular, $G_{\aaa\mapsto \aaa} = G_\aaa$. Clearly $G_{\aaa_0 \mapsto \aaa_1}$ is a right coset of $G_{\aaa_0}$ and a left coset of $G_{\aaa_1}$. Also $G_{\aaa_1 \mapsto \aaa_0}= G_{\aaa_0 \mapsto \aaa_1}^{-1}$. We extend \cref{fac2}(i). 
 
   \begin{fact}  \label{fac3}
  
       $G_{\aaa_0 \mapsto \aaa_1}=:A  \sub B:= G_{\beta_0 \mapsto \beta_1}  \LR $
       
       \hfill $A = \ES \vee \beta_i \in \text{dcl}(\aaa_i)$ ($i=0,1)$ via the same formula. \end{fact}
  \begin{proof}
 (i) The implication ``$\LA$'' is again  immediate. For ``$\RA$", suppose $\aaa_i = \ol a_i /E$ and $\beta_i = \ol b_i /F$ as above. Since $G_{\aaa_0} \sub G_{\beta_0}$, as before we have $\beta_0 \in \text{dcl}(\aaa_0)$, say via formula $\phi(\ol x, \ol y)$. 
 We may assume $A \neq \ES$, that is there is $g\in G$ with $g (\aaa_0) = \aaa_1$. Then $g (\beta_0) = \beta_1$. Hence $\beta_1 \in \text{dcl}(\aaa_1)$ via $\phi$. \end{proof}
 
 
 
 
 \subsubsection{Meet groupoid operations}
 
 
